Compositional Generalization in Dependency Parsing

Compositionality -- the ability to combine familiar units like words into novel phrases and sentences -- has been the focus of intense interest in artificial intelligence in recent years. To test compositional generalization in semantic parsing, Keysers et al. (2020) introduced Compositional Freebase Queries (CFQ). This dataset maximizes the similarity between the test and train distributions over primitive units, like words, while maximizing the compound divergence: the dissimilarity between test and train distributions over larger structures, like phrases. Dependency parsing, however, lacks a compositional generalization benchmark. In this work, we introduce a gold-standard set of dependency parses for CFQ, and use this to analyze the behavior of a state-of-the art dependency parser (Qi et al., 2020) on the CFQ dataset. We find that increasing compound divergence degrades dependency parsing performance, although not as dramatically as semantic parsing performance. Additionally, we find the performance of the dependency parser does not uniformly degrade relative to compound divergence, and the parser performs differently on different splits with the same compound divergence. We explore a number of hypotheses for what causes the non-uniform degradation in dependency parsing performance, and identify a number of syntactic structures that drive the dependency parser's lower performance on the most challenging splits.

==> Compositional Generalization in Dependency Parsing/figs/FPTRHC.tex <==
    \begin{figure}[t]  
\centering  

\includegraphics[width = \linewidth, keepaspectratio]{figs/FPTRHCFigure.pdf} 
 
 \caption{An example question from the CFQ dataset, with the associated SPARQL query and dependency parse.}  
\label{fig:fptrhc}  
\end{figure}  

==> Compositional Generalization in Dependency Parsing/figs/divergenceLengths.tex <==
\begin{figure}[ht]
    \centering
    \includegraphics[width = .45\textwidth]{figs/divergenceLengthsFigure.pdf}
    
    \caption{Divergence between test and train of the MCD and random splits. Roughly, divergence increases with subtree complexity, although much more rapidly for MCD splits than random. Additionally, there is little difference between the different MCD splits.}
    \label{fig:divergenceLengths}
\end{figure}

==> Compositional Generalization in Dependency Parsing/figs/errormatrices.tex <==
\begin{figure}[h]
\includegraphics[width=.23\textwidth]{figs/errorMatrix_MCD1.pdf}
\includegraphics[width=.23\textwidth]{figs/errorMatrix_MCD3.pdf}
\caption{Percentage of the test set which is correctly parsed by five semantic parsing experiments and five dependency parsing experiments, for MCD1 and MCD3.}
\label{fig:errormatrices}
\end{figure}

==> Compositional Generalization in Dependency Parsing/figs/fewshotLengths.tex <==
\begin{figure}[ht]
    \includegraphics[width = .45\textwidth,keepaspectratio]{figs/fewshotLengthsFigure.pdf}
    \caption{The proportion of syntactic constructions in test which appear in train fewer than four times, for all subtree complexities. Complexity is measured in number of arcs.}
    \label{fig:fewshotLengths}
\end{figure}

==> Compositional Generalization in Dependency Parsing/figs/scatterplot.tex <==
\begin{figure}[ht]
    \includegraphics[width = .45\textwidth, keepaspectratio]{figs/scatterplotFigure.pdf}
    \caption{The effect of compound divergence on Content-word Labeled Attachment Score (CLAS) and Whole-Sentence Content Labeled Attachment Score (WSCLAS).}
    \label{fig:scatterplot}
\end{figure}

==> Compositional Generalization in Dependency Parsing/figs/subtrees.tex <==
\begin{figure}[ht]
    \includegraphics[width = .5\textwidth, keepaspectratio]{figs/SubtreesFigure.pdf}
    \caption{A dependency parse and two of its subtrees}
    \label{fig:subtrees}
\end{figure}

==> Compositional Generalization in Dependency Parsing/figs/untrainedLengths.tex <==
\begin{figure}[ht]
    \includegraphics[width = .45\textwidth, keepaspectratio]{figs/untrainedLengthsFigure.pdf}
    \caption{The proportion of syntactic constructions in test which are untrained, for all splits and all subtree complexities. Subtree complexity is measured in number of arcs.}
    \label{fig:untrainedLengths}
\end{figure}

==> Compositional Generalization in Dependency Parsing/tables/badTrees.tex <==
\begin{table*}[h!t]
\vspace{.5cm}
\small
\centering
\begin{tabular}{lllllllllll}
\toprule
 Tree &  MCD1 &       &       &    MCD2 &       &       &  MCD3 &       &    &     \\
    &  Train \# & Test \# & $\Delta \%$  & Train \# & Test \# & $\Delta \%$ & Train \# & Test \# & $\Delta \%$ &   \\
\midrule
& \multicolumn{9}{c}{Predictive for MCD1} \\
\resizebox{!}{.5in}{
\begin{dependency}
\begin{deptext}
and \& entity \& verb \\ % VERB, ((CC, and), (NSUBJ, entity) 
\end{deptext} 
\depedge{3}{1}{{\small CC}}
\depedge{3}{2}{{\small NSUBJ}}
\deproot[edge unit distance=2ex]{3}{root}
\end{dependency}}& 2342 & 192   & 0.26  & 2099 & 144   & -0.15 & 1546 & 118   & 0.01  \\ %1 
 
 \resizebox{!}{.5in}{
\begin{dependency} %entity, ((CASE, of), (CONJ, entity), (CONJ, entity), (CONJ, entity))
\begin{deptext}
of \& entity \& entity \& entity \& entity \\
\end{deptext}

\depedge{2}{1}{{\small CASE}}
\depedge{2}{3}{{\small CONJ}}
\depedge{2}{4}{{\small CONJ}}
\depedge{2}{5}{{\small CONJ}}
\deproot[edge unit distance=2ex]{2}{root}
\end{dependency}}& 0    & 484   & 1.29  & 0    & 405   & -0.15 &  0    & 382   & 1.78  \\ % 1

\resizebox{!}{.5in}{
 \begin{dependency} % np_simple, ((AMOD, adjective_simple), (CASE, "s")
\begin{deptext}
adjective \& noun \&  's \\
\end{deptext}

\depedge{2}{1}{{\small AMOD}}
\depedge{2}{3}{{\small CASE}}
\deproot[edge unit distance=2ex]{2}{root}

\end{dependency} } & 2319 & 137   & 0.23 & 3033 & 3     & -0.0  & 3255 & 50    & -0.1  \\ %1

\midrule
& \multicolumn{9}{c}{Predictive for MCD2 and MCD3} \\

\resizebox{!}{.5in}{
\begin{dependency} % role_simple, ((COP, was), (NSUBJ, role_simple))
\begin{deptext}
was \& role \& role \\
\end{deptext}

\depedge{3}{1}{{\small COP}}
\depedge{3}{2}{{\small NSUBJ}}
\deproot[edge unit distance=2ex]{3}{root}
\end{dependency}} & 367  & 792   & -0.0  & 0    & 940   & 5.73  &  0    & 1437  & 6.98   \\ % 2,3

\resizebox{!}{.5in}{
\begin{dependency} % role_simple, ((COP, was), (NSUBJ, noun_simple))
\begin{deptext}
was \& noun \& role \\
\end{deptext}

\depedge{3}{1}{{\small COP}}
\depedge{3}{2}{{\small NSUBJ}}
\deproot[edge unit distance=2ex]{3}{root}
\end{dependency}} & 0    & 530   & -0.06  & 0    & 535   & 2.25  & 0    & 593   & 0.54   \\ % 2 3

\resizebox{!}{.5in}{
\begin{dependency} %np_simple, ((NSUBJ, role_simple), (DET, a))
\begin{deptext}
role \& a \& noun \\
\end{deptext}

\depedge{3}{1}{{\small NSUBJ}}
\depedge{3}{2}{{\small DET}}
\deproot[edge unit distance=1.5ex]{3}{root}

\end{dependency}} & 0    & 541   & 0.02   & 0    & 547   & 2.38  & 0    & 604   & 2.01 \\ %2 3 

\resizebox{!}{.5in}{
\begin{dependency} % vp_simple, ((AUX, was), (NSUBJ, np_simple))
\begin{deptext}
was \& noun \& verb \\
\end{deptext}
\depedge{3}{1}{{\small AUX}}
\depedge{3}{2}{{\small NSUBJ}}
\deproot[edge unit distance=2ex]{3}{root}

\end{dependency}} & 872  & 60  & -0.02  & 0    & 512   & 2.94  &  0    & 547   & 2.61 \\ %2 3

\resizebox{!}{.5in}{
\begin{dependency} % vp_simple, ((AUX, was), (NSUBJ, role_simple))
\begin{deptext}
was \& role \& verb \\
\end{deptext}
\depedge{3}{1}{{\small AUX}}
\depedge{3}{2}{{\small NSUBJ}}
\deproot[edge unit distance=1.75ex]{3}{root}
\end{dependency}} & 1484 & 231   & -0.03 & 0    & 993   & 2.53  &  0    & 1093  & 3.06 \\%2 3

\midrule
& \multicolumn{9}{c}{Predictive for MCD3} \\

\resizebox{!}{.5in}{
\begin{dependency} %vp_simple, ((CONJ, vp_simple), (OBJ, entity), (PUNCT, ?))
\begin{deptext}
verb \& verb \& entity \& ? \\
\end{deptext}

\depedge{1}{4}{{\small PUNCT}}
\depedge{1}{3}{{\small OBJ}}
\depedge{1}{2}{{\small CONJ}}
\deproot[edge unit distance=2ex]{1}{root}

\end{dependency}} & 877  & 1513  & 0.1  & 451  & 1435  & -2.53 & 355  & 1407  & 1.47 \\ % 3

\resizebox{!}{.5in}{
\begin{dependency} %entity, ((CASE, of), (CONJ, entity), (CONJ, entity))
\begin{deptext}
of \& entity \& entity \& entity \\
\end{deptext}

\depedge{2}{1}{{\small CASE}}
\depedge{2}{4}{{\small CONJ}}
\depedge{2}{3}{{\small CONJ}}
\deproot[edge unit distance=1.75ex]{2}{root}

\end{dependency}} & 0    & 1153  & 1.33 & 509  & 905   & -0.97 & 0    & 931   & 3.95 \\ %3
\bottomrule
\end{tabular}
\caption{Syntactic constructions most predictive of dependency parsing failure for each split. ``Predictive'' means the subtree is associated with a coefficient $\leq -1$ by the logistic model. \# stands for the number of occurrences. $\Delta \%$ is defined as the change in mean WSCLAS after all instances of the construction have been removed from test. \label{tbl:badTrees}}
\vspace{.3cm}
\end{table*}




==> Compositional Generalization in Dependency Parsing/tables/dataset_statistics.tex <==
\begin{table}[ht]
\centering
\resizebox{\linewidth}{!}{
\begin{tabular}{c c c c c}
\toprule
& \multicolumn{2}{c}{Total Sentences} & \multicolumn{2}{c}{Unique Constructions} \\
 & Train & Test & Train & Test\\
\midrule
MCD1  & 76,595 & 11,968 & 2,093 & 2,048 \\
\rowcolor{gray!6} MCD2  & 76,595 & 11,967 & 2,006 & 1,884 \\
MCD3 & 76,595 & 11,968 & 2,300 & 1,823 \\
\rowcolor{gray!6} Random & 76,596 & 11,967 & 4,082 & 3,251\\
\bottomrule
\end{tabular}}
\caption{Number of sentences and unique constructions for each test and train set in our experiments (see \textsection~\ref{sec:constructions} for an explanation of constructions). 
\label{tbl:dataset_statistics}}
\end{table}

==> Compositional Generalization in Dependency Parsing/tables/mcd_scores.tex <==
\begin{table}[ht]
\centering
\resizebox{\linewidth}{!}{
\begin{tabular}{c c c c c}
\toprule
& \multicolumn{3}{c}{Dependency Parser} & Semantic Parser\\
Split & WSCLAS & CLAS & LAS & Exact Match\\
& \small{mean (sd)} & \small{mean (sd)} & \small{mean (sd)} & \small{mean ($95\%$ conf interval)}\\
\midrule
MCD1 & 96.57 $\pm{1.31}$ & 99.38 $\pm{0.29}$ & 99.64 $\pm{0.16}$& 37.4 $\pm{2.2}$\\
\rowcolor{gray!6} MCD2 & 71.42 $\pm{2.59}$& 91.53  $\pm{1.00}$ & 93.28 $\pm{0.88}$& 8.1$\pm{1.6}$\\
MCD3 & 56.76 $\pm{2.81}$ & 87.66  $\pm{0.93}$ & 90.87 $\pm{1.01}$&11.3 $\pm{0.3}$ \\
\rowcolor{gray!6} Random & 99.89 $\pm{0.01}$ & 99.98$\pm{0.00}$ & 99.99 $\pm{0.00}$& 98.0 $\pm{0.3}$\\
\bottomrule
\end{tabular}}
\caption{Stanza's performance on MCD splits in terms of Whole Sentence Content-word Labeled Attachment Score (WSCLAS), Content-word Labeled Attachment Score (CLAS), and Labeled Attachment Score (LAS). Means and standard deviations are calculated over five randomly-seeded runs. The semantic parsing scores are reproduced from \citep{keysers2020measuring}; the mean exact-match of 5 experiments with $95\%$ confidence intervals is reported for each MCD split in their github repository.\footnote{https://github.com/google-research/google-research/tree/master/cfq}
\label{tbl:mcd_scores}}
\end{table}









==> Compositional Generalization in Dependency Parsing/tables/reducedTestSetScores.tex <==
\begin{table*}[htb]
\centering
\resizebox{0.8\textwidth}{!}{
\begin{tabular}{ccccccc}
\toprule
 Split & Num Trees & Sentences in & WSCLAS, StDv         & CLAS, StDv           & LAS, StDv            & Num Sentences \\
       & removed & reduced test &                      &                      &                      & removed      \\
\midrule
 mcd1  & 3 & 11,139        & 98.41 $\pm$0.71  & 99.75  $\pm$0.15 & 99.84$\pm$0.1 & 828           \\
\rowcolor{gray!6} mcd2 & 5 & 8,440         & 92.46 $\pm$3.82 & 98.59$\pm$0.47 & 98.89$\pm$0.37 & 3527                     \\
mcd3 & 7 & 5,692         & 93.09$\pm$2.77  & 98.79$\pm$0.50    & 98.91$\pm$0.36 & 6275        \\
\rowcolor{gray!6} rand  & 0 & 11,967        & 99.89$\pm$0.01  & 99.98  $\pm$0.00  & 99.99 $\pm$0.00 & 0           \\
\bottomrule
\end{tabular}}
\caption{Re-calculated accuracy on the test sets, when removing all sentences whose subtrees are most predictive of Stanza's failure.\label{tbl:reducedTestSetScores}}
\end{table*}



